Stability of Axion-Saxion wormholes

We reconsider the perturbative stability of Euclidean axion wormholes. The quadratic action that governs linear perturbations is derived directly in Euclidean gravity. We demonstrate explicitly that a stability analysis in which one treats the axion as a normal two-form gauge field is equivalent to one performed in the Hodge-dual formulation, where one considers the axion as a scalar with a wrong-sign kinetic term. Both analyses indicate that axion wormholes are perturbatively stable, even in the presence of a massless dilaton, or saxion, field that couples to the axion.

==> appendices/perturbation_theory.tex <==
\section{Perturbation theory}\label{pert appendix}
We consider the action in the three-form field strength form, viz.
\begin{align}
\label{eqn:action-field-strength-three-form}
S_E &= \int \dd[4]{x} \sqrt{g} \left( - \frac{1}{2} \Rs + \frac{1}{12} e^{-b \ph} \Ft{_{\mu\nu\sigma}} \Ft{^{\mu\nu\sigma}} + \frac{1}{2} \CD{_\mu} \ph \CD{^{\mu}} \ph + \frac{1}{6} \chi \eps{^{\mu\nu\rho\sigma}} \CD{_\mu} \Ft{_{\nu\rho\sigma}} \right),
\end{align}
and in the scalar field formulation
\begin{align}
\label{eqn:action-field-scalar}
S_E &= \int \dd[4]{x} \sqrt{g} \left( - \frac{1}{2} \Rs - \frac{1}{2} e^{b \ph} \CD{_\mu} \chi \CD{^\mu} \chi + \frac{1}{2} \CD{_\mu} \ph \CD{^\mu} \ph + \CD{_\mu} \left( e^{b\ph} \chi \CD{^\mu} \chi \right) \right).
\end{align}
We expand the action to quadratic order in the perturbations using the Mathematica package $x$Pand \cite{Pitrou:2013hga}, which
uses the tensor algebra package $x$Tensor in the $x$Act distribution \cite{Martin:2008xtensor} together with the package $x$Pert,
for perturbations \cite{Brizuela:2008ra}.\footnote{For this the $x$Pand package was modified to calculate
conformal perturbations in Euclidean instead of Lorentzian spacetime \cite{Maenaut:2020Git}.}
The perturbed Euclidean Einstein-Hilbert action reads,
%is perturbed to second order, where, up to a total derivative, all the remaining terms are the product of two first-order perturbations that form the quadratic action given by
\begin{comment}
\begin{align}
\delta^2 S_E^\text{gr.} = - &\frac{1}{2} \int \dd[4]{x} \sqrt{\gt{}} \Bigg[ \frac{1}{4} \left( \CD{_\mu} \dg{^\nu_\nu} \right) \left( \CD{^\mu} \dg{^\lambda_\lambda} \right)
 - \frac{1}{2} \left( \CD{^\mu} \dg{^\lambda_\lambda} \right) \left( \CD{_\nu} \dg{_\mu^\nu}\right) + \frac{1}{2} \left( \CD{_\mu} \dg{_{\lambda\nu}} \right) \left( \CD{^\nu} \dg{^{\lambda\mu}} \right)
  \notag\\ 
&- \frac{1}{4} \left( \CD{_\nu} \dg{_{\lambda\mu}} \right) \left( \CD{^\nu} \dg{^{\lambda\mu}} \right) + \dg{_\alpha^\nu} \dg{^{\alpha\mu }} \Rt{_{\mu\nu}}
 - \frac{1}{2} \dg{^\alpha_\alpha} \dg{^{\mu\nu}} \Rt{_{\mu\nu}}
 - \frac{1}{4} \dg{_{\alpha\mu}} \dg{^{\alpha\mu}} \Rs
 + \frac{1}{8} \dg{^\alpha_\alpha} \dg{^\mu_\mu} \Rs \Bigg] .
\end{align}
Note that second-order perturbations of the metric and the fields are disregarded as they are multiplied with background expressions in the perturbed action that are zero due to the equations of motion. Selecting the scalar perturbations, we fill in the metric fluctuation from \eqref{eqn:scalar-metric-perturbation}, which yield, 
\end{comment}
up to a total derivative in $r$ and a covariant total derivative on the induced metric, 
%the following quadratic action
\begin{align}
\delta^2 S_E^\text{gr.} =& - \frac{1}{2} \int \dd{r} \dd[3]{x} \Big( a^2 \sqrt{\gamma} \Big[
  \Big(
   6 \left( \dpsid \right)^2
 + 12\Hh \left( \dA + \dpsi \right) \dpsid
 + 9 \Hh^2 \left( \dA + \dpsi \right)^2
 + 4 \Hh \left( \dA + \dpsi \right) \triangle \left( \dB - \dEd \right)
 - 4 \Hh \dpsid \triangle \dE \notag\\
&+ 4 \dpsid \triangle \left( \dB - \dEd \right)
 + 4 \Hh \cd{_i} \dpsi \cd{^i} \dB
 - 6 \Hh^2 \left( \dA + \dpsi \right) \triangle \dE 
 + 4 \Hh \triangle \dE \triangle \left( \dB - \dEd \right)
 - 4 \Hh \triangle E \triangle B
 - 3 \Hh^2 \left( \triangle E \right)^2 \Big)\notag\\
&+ 3 \Hh^2 \cd{_i} \dB \cd{^i} \dB
 - 2 \cd{^i} \dpsi \cd{_i} \left( 2 \dA - \dpsi \right)
 - \kh \Big(
 + 3 ( \dA + \dpsi )^2
 + 2 \, (\dB - \dEd) \triangle (\dB - \dEd)
 - (6 \dA - 2\dpsi + \triangle \dE)  \triangle \dE\notag\\
&+ 3 \,  (\cd{_i} \dB)(\cd{^i} \dB)
 + 4 \,  ( \Hhd+\Hh^2) (\cd{_i} \dE)(\cd{^i} \dE)
 + 2 (\cd{_j} \cd{_i} \dE)(\cd{^j} \cd{^i} \dE)
  \Big)
\Big]\Big).
\end{align}
%where $k$ is linked to the curvature of the induced three-dimensional metric. 
For $k=0$, this agrees with the calculations in \cite{Mukhanov:1992me} after Wick rotation and up to the above-mentioned total derivatives.

% 3.2
% (axion + dilaton) both the scalar and three form approach

% dilaton sector perutbation

\begin{comment}
For the field sector of the action, we start with the second-order perturbation of the dilaton term, which is simply a free scalar field. We perturb the metric and the dilaton field, which yields the following quadratic action
\begin{align}
\delta^2 S_E^\text{dilaton} = \int \dd[4]{x} \sqrt{\gt{}} \bigg(&
   \left( -\frac{1}{8} \dg{_{\beta\gamma}} \dg{^{\beta\gamma}}
 + \frac{1}{16} \dg{^\beta_\beta} \dg{^\gamma_\gamma} \right)
\left( \CD{_\alpha} \ph \CD{^\alpha} \ph \right)
 + \frac{1}{2} \dg{^\beta_\beta} \CD{_\alpha} \dph \CD{^\alpha} \ph
 + \frac{1}{2} \CD{_\alpha} \dph \CD{^\alpha} \dph \notag\\
&- \dg{_{\alpha\beta}} \CD{^\alpha} \ph \CD{^\beta} \dph
 + \left( \frac{1}{2} \dg{_\alpha^\gamma} \dg{_{\beta\gamma}}
 - \frac{1}{4} \dg{_{\alpha\beta}} \dg{^\gamma_\gamma} \right)
   \left( \CD{^\alpha} \ph \CD{^\beta} \ph \right) \bigg) .
\end{align}
%
If we select the scalar perturbations of the metric fluctuation \eqref{eqn:scalar-metric-perturbation}, this yields, 
\end{comment}
The perturbed dilaton-field sector of the action is given by, again up to a total derivative in $r$ and a total derivative on the induced metric, 
%the following quadratic action
\begin{align}
\delta^2 S_E^\text{dilaton} = \int& \dd{r} \dd[3]{x} \,  a^2 \sqrt{\gamma}  \, \bigg[
   \frac{1}{2} \left( \dphd^2  + \cd{_i} \dph \cd{^i} \dph \right)
 - \phd \left( \dphd \left( \dA + 3 \dpsi - \triangle \dE \right)
 + \cd{_i} \dph \cd{^i} \dB \right) \notag \\
&+ \frac{1}{4} \phd^2 \left( 3 \dA^2 + 3 \dpsi^2 + 6\dA \dpsi
 - 2 \dpsi \triangle \dE -2 \dA \triangle \dE
 + \cd{_i} \dB \cd{^i} \dB
 + \triangle \dE \triangle \dE
 - 2 \cd{_i} \cd{_j} \dE \cd{^i} \cd{^j} \dE \right)
 \bigg] .
\end{align}

%\newpage

For the axion field, it is useful to demonstrate explicitly that the perturbed action derived from \eqref{eqn:action-field-strength-three-form} is equivalent to the one derived from \eqref{eqn:action-field-scalar}. Starting with the former, the perturbed action up to quadratic order in the perturbations is given by
\begin{align}\label{eqn:perturbed-three-form-field-strength-axion-action}
\delta^2 S_E^\text{axion} &= \int \dd[4]{x} \sqrt{g} \bigg[ e^{-b \ph} \bigg( 
  \frac{1}{12} \dF{^{\mu\nu\rho}} \dF{_{\mu\nu\rho}}
 + \frac{1}{12} \dg{^\alpha_\alpha} \Ft{^{\mu\nu\rho}} \dF{_{\mu\nu\rho}}
 - \frac{1}{2} \dg{^{\alpha\beta}} \Ft{^{\mu\nu}_\alpha} \dF{_{\mu\nu\beta}}
 + \frac{1}{4} \dg{^{\alpha\beta}} \dg{^{\kappa\lambda}} \Ft{^{\mu}_{\alpha\kappa}} \Ft{_{\mu\beta\lambda}} \notag\\
&+ \frac{1}{4} \left( \dg{^{\alpha\sigma}} \dg{_\sigma^\beta} - \frac{1}{2} \dg{^\sigma_\sigma} \dg{^{\alpha\beta}} \right)
   \Ft{^{\mu\nu}_\alpha} \dF{_{\mu\nu\beta}}
 + \frac{1}{48} \left( \frac{1}{2} \dg{^\alpha_\alpha} \dg{^\beta_\beta} - \dg{^{\alpha\beta}} \dg{_{\alpha\beta}} \right)
   \Ft{^{\mu\nu\rho}} \Ft{_{\mu\nu\rho}}
   + \frac{1}{24} b^2 \dph^2 \Ft{^{\mu\nu\rho}} \Ft{_{\mu\nu\rho}} \notag\\
&- b \dph \left( 
   \frac{1}{6} \Ft{^{\gamma\mu\nu}} \dF{_{\gamma\mu\nu}}
 + \frac{1}{24} \dg{^\gamma_\gamma} \Ft{^{\mu\nu\alpha}} \Ft{_{\mu\nu\alpha}}
 - \frac{1}{4} \dg{^{\gamma\mu}} \Ft{_\gamma^{\nu\alpha}} \Ft{_{\mu\nu\alpha}}  
  \right) \bigg)
 + \frac{1}{6} \eps{^{\alpha\mu\nu\rho}} \dch \CD{_\alpha} \dF{_{\mu\nu\rho}}
\bigg]
\end{align}
As in \eqref{eq: Hodge}, we can integrate the last term by parts and apply the equations of motion for the field strength fluctuation to find a Hodge-dual relation expanded to first order in the perturbation: 
%(indices of $F$ have to be lowered when perturbing)
\begin{align}\label{eqn:perturbed-hodge-duality}
\Ft{_{\mu\nu\rho}} &= e^{b \ph} \eps{_{\sigma\mu\nu\rho}} \CD{^\sigma} \chi, \\
\dF{_{\mu\nu\rho}} &= e^{b \ph} \eps{_{\sigma\mu\nu\rho}} \left( b\,\dph \CD{^\sigma} \chi + \CD{^\sigma} \dch + \frac{1}{2} \dg{^\alpha_\alpha} \CD{^\sigma} \chi - \dg{^{\sigma\beta}} \CD{_\beta} \chi \right).
\end{align}
% where we note that the indices of the field strength have to be lowered when applying a perturbation.
% Notice that the first order expression contains the same information as the equation of motion for $\dF{}$ derived from the action above. 

Starting with the scalar-field formulation of the axion action \eqref{eqn:action-field-scalar}, the second-order perturbed action reads
%ation and keep the first-order perturbations of  the metric and the fields, the quadratic action equals
\begin{align}\label{eqn:perturbed-scalar-field-axion-action}
\delta^2 S_E^\text{axion} =  \int \dd[4]{x} \sqrt{\gt{}} \bigg[& e^{b\ph} \bigg(
   \left( \frac{1}{4} \dg{_{\alpha\beta}} \dg{^\gamma_\gamma}
 - \frac{1}{2} \dg{_\alpha^\gamma} \dg{_{\beta\gamma}} \right)
   \left( \CD{^\alpha} \chi \CD{^\beta} \chi \right) 
 + \left( \frac{1}{8} \dg{_{\beta\gamma}} \dg{^{\beta\gamma}}
 - \frac{1}{16} \dg{^\beta_\beta} \dg{^\gamma_\gamma} \right)
   \left( \CD{_\alpha} \chi \CD{^\alpha} \chi \right)\notag\\
&- \frac{1}{2} \CD{_\alpha} \dch \CD{^\alpha} \dch 
 - \frac{1}{2} \dg{^\beta_\beta} \CD{_\alpha} \dch \CD{^\alpha} \chi
 + \dg{_{\alpha\beta}} \CD{^\alpha} \chi \CD{^\beta} \dch \notag\\
&+ b \dph \left( \frac{1}{2} \dg{_{\alpha\beta}} \CD{^\alpha} \chi \CD{^\beta} \chi
 - \frac{1}{4} \dg{^\alpha_\alpha} \CD{_\beta} \chi \CD{^\beta} \chi
 - \CD{_\alpha} \chi \CD{^\alpha} \dch \right)
 - \frac{1}{4} b^2 \dph^2 \CD{^\alpha} \chi \CD{_\alpha} \chi \notag \bigg)  \\
&+ \CD{_\mu} \bigg(e^{b\ph}\Big(
(\dg{_{\alpha \beta}} \dg{^{\mu \beta}} \chi \CD{^\alpha} \chi
-  \dg{^\mu_\alpha} \left( \dch \CD{^\alpha} \chi + \chi \CD{^\alpha} \dch \right) 
+ \dch \CD{^\mu}\dch)
- \frac{1}{2} \dg{^\beta_\beta} \dg{^\mu_\alpha} \chi \CD{^\alpha} \chi \notag\\
&- \frac{1}{4} \dg{_{\alpha\beta}} \dg{^{\alpha\beta}} \chi \CD{^\mu} \chi
+ \frac{1}{8} \dg{^\alpha_\alpha} \dg{^\beta_\beta} \chi \CD{^\mu} \chi
+ \frac{1}{2} \dg{^\alpha_\alpha} \left( \dch \CD{^\alpha} \chi + \chi \CD{^\alpha} \dch \right) \notag\\
&
+ b\dph(\chi \CD{^\mu} \dch - \dg{^\mu^\alpha} \chi \CD{_\alpha} \chi + \frac{1}{2} \dg{^\alpha_\alpha} \chi \CD{_\mu} \chi + \dch \CD{^\mu} \chi)
+\frac{1}{2} b^2 \dph^2 \chi \CD{^\mu}\chi\Big)\bigg)\bigg]
\end{align}
where the last three lines come from the boundary term. Equivalently, this can be obtained by inserting \eqref{eqn:perturbed-hodge-duality} in \eqref{eqn:perturbed-three-form-field-strength-axion-action}. 
%obtain the quadratic action associated with the scalar field formulation of the axion in \eqref{eqn:perturbed-scalar-field-axion-action} above, 
\footnote{Note that this requires keeping all contributions of the second-order perturbations of $\Ft{_{\nu\rho\sigma}}$ that contain products of $\dg{_{\mu\nu}}$ and the scalars $\dch, \dph$, which form a total derivative. Also, although contributions of $\delta^2 \Ft{_{\nu\rho\sigma}}$ are multiplied with background expressions that are zero, these are needed to show the equivalence of the perturbed action under the Hodge duality, since these lead to terms that include the product of two first-order perturbations.}

Expressing the three-form fluctuations as in \eqref{eqn:perturbed-three-form} and restricting to the scalar metric perturbations of \eqref{eqn:scalar-metric-perturbation}, the quadratic action \eqref{eqn:perturbed-three-form-field-strength-axion-action}, up to a total derivative on the induced metric, becomes
\begin{align}
\delta^2 S_E^{F} = \int \dd{r} \dd[3]{x} \, \frac{\sqrt{\gamma}}{a^2} \bigg[& e^{-b \ph} \bigg( 
\frac{1}{2} \left( f^2 + \cd{_i} w \cd{^i} w \right) + Q \left( f \left( \dA + 3 \dpsi - \triangle \dE - b \dph  \right) + w \triangle \dB \right)\notag\\
&- \frac{1}{4} Q^2 \Big( 2 b \dph \left( \dA + 3 \dpsi - \triangle \dE \right) - b^2 \dph^2 + \dA^2 - 15 \dpsi^2  - 6 \dA \dpsi + 2 \dB \triangle \dB + 2 \dA \triangle \dE\notag\\
&+ 10 \dpsi \triangle \dE + \cd{_i} \dB \cd{^i} \dB - \triangle \dE \triangle \dE - 2 \cd{_i} \cd{_j} \dE \cd{^i} \cd{^j} \dE  \Big) \bigg)
 + 4 a^2 \dch \left( \Dot{f} - \triangle w \right) \bigg].
\end{align}
Likewise, the scalar form of the perturbed axion action \eqref{eqn:perturbed-scalar-field-axion-action}, excluding the final boundary term, equals
%restricted to axion fluctuations and select the scalar perturbations of the metric, the quadratic action in \eqref{eqn:perturbed-scalar-field-axion-action}, 
\begin{align}
\delta^2 S_E^{\chi} = \int \dd{r} \dd[3]{x} \, a^2 \sqrt{\gamma}  e^{b\ph} \Big(&
\chid \left( \dchd \left( \dA + 3 \dpsi - \triangle \dE - b \dph \right) + \cd{_i} \dch \cd{^i} \dB \right)
- \frac{1}{2} \left( (\chid)^2 + \cd{_i} \chi \cd{^i} \chi \right) \notag\\
& - \frac{1}{4} (\chid)^2 \big( 2 b \dph \left( \dA + 3 \dpsi - \triangle \dE \right) + b^2 \dph^2 + 3 \dA^2 + 3 \dpsi^2 + 6 \dA \dpsi \notag\\
&- 2 \dpsi \triangle \dE  -2 \dA \triangle \dE + \cd{_i} \dB \cd{^i} \dB + \triangle \dE \triangle \dE - 2 \cd{_i} \cd{_j} \dE \cd{^i} \cd{^j} \dE \big)
\Big) .
\end{align}
Now, adding the boundary term contributions 
%that are a product of first order perturbations of the metric $\dg{_{\mu\nu}}$ and scalars $\dch, \dph$ 
and subtracting the contributions from the second-order perturbations $\Ft{_{\nu\rho\sigma}}$, we find that the difference is given by
% subtract the total derivative $\CD{_\mu} \left( \chi \, \eps{^{\mu\nu\rho\sigma}}\,  \delta^{(2)} \tensor{F}{_{\nu\rho\sigma}} \right) $
\begin{align}
\delta^2 S_E^\text{boundary} = \int \dd{r} \dd[3]{x} \, a^2 \sqrt{\gamma}  e^{b\ph} \Big(
(\dchd)^2 - \chid \dchd \left( \dA + 3 \dpsi -\triangle \dE \right) - \chid \cd{_i} \dch \cd{^i} \dB + \cd{_i} \dch \cd{^i} \dch
 + b \dph \chid \dchd
\Big).
\end{align}
Hence both formulations are equivalent through the following transformations derived from the Hodge duality rules \eqref{eqn:perturbed-hodge-duality}
\begin{align}\label{transformations axion}
\chid &\to \frac{e^{-b \ph} Q}{a^2},&
\dchd &\to \frac{e^{-b \ph}}{a^2} \left( f + Q \left( \dA + 3 \dpsi - \triangle \dE - b\dph \right) \right),
& \cd{_i} \dch &\to \frac{e^{-b \ph}}{a^2} \left( \cd{_i} w + Q \cd{_i} \dB \right) .
\end{align}

\subsection{Constraints and gauge invariance}\label{Gaugeinvformalism}
% 3.3
% Gauge invariant variables, boundary conditions and field equivalence
\subsubsection{The three-form formulation}
After imposing the closure of $F$, i.e. replacing $w$ with $\Dot{f}/\triangle$, the resulting quadratic action is given by:
% Bruno's Thesis 5.17
% ACTION OF f and w, A, B, E, psi, ph, chi EIGHT scalar dof
\begin{align}
\delta^2 S_E = \int \dd{r} \dd[3]{x} \, \sqrt{\gamma} \bigg[ \frac{e^{-b\ph}}{a^2} \Big(&
\frac{1}{2} \left( f^2 - (\Dot{f})^2/\triangle \right) 
+ Q \left( f \left(\dA + 3 \dpsi - \triangle \dE -b \dph \right) + \dB \Dot{f} \right)
+ \frac{1}{4} Q^2 b^2 \dph^2 \notag\\
&+ \frac{1}{2} Q^2 \left(
\left( \dA + 3 \dpsi - \triangle \dE \right)^2
- b \dph \left( \dA + 3 \dpsi - \triangle \dE \right)
- \dB \triangle \dB + \dB \Dot{f}
\right)
\Big)
\notag\\
&+a^2 \Big( \frac{1}{2} \left( (\dphd)^2 - \dph \triangle \dph \right)
+ \phd \dph \left(3 \dpsid + \triangle \left( \dB - \dEd \right) \right) - \dA \phd \dphd \notag\\
&+ \dpsi \triangle \left(\dpsi - 2 \dA \right)
- 3 (\dpsid)^2 - 6 \Hh \dA \dpsid - 2 \left( \Hh \dA + \dpsid \right) \triangle \left( \dB - \dEd\right) \notag\\
&+ \kh \left( 3\dpsi^2 - 6 \dA \dpsi - 3 \dA^2 + \left(\dB - \dEd \right)\triangle \left(\dB - \dEd \right) \right)
\Big)
\bigg]
\end{align}
Again, note that we found this action with the background field equations and an expansion into spherical harmonics.
%
To find the constraints set by the non-dynamical variables $\dA$ and $\dB$, which act as Lagrange multipliers in the action, we write the quadratic action using the Hamiltonian formalism
\begin{align}
S = \int \dd{r} \left[ p_i \Dot{q}_i - H(p,q) - C_i G^i(p,q)  \right],
\end{align}
where $C_i$'s are the Lagrange multipliers and $G^i(p,q)$ are the constraints they impose.

The conjugate momenta of the dynamical variables $\dpsi, \dE, f \text{ and } \dph$ are given by
\begin{align} % Bruno's Thesis 5.19
\Pf &= \frac{e^{-b\ph}}{\triangle a^2} \left( Q \triangle \dB - \Dot{f} \right),& \Ppsi &= a^2 \left(3 \phd \dphd - 6 \dA \Hh - 6 \dpsid +  2 \triangle\left( \dEd - \dB \right) \right), \notag\\
\Pdph &= a^2 \left( \dphd - \phd \dA \right),& \PE &= \triangle a^2 \left( - \phd \dphd + 2 \dA \Hh + 2 \dpsid + 2 \kh \left( \dEd - \dB \right) \right).
\end{align}
These can be substituted into the action to write it in Hamiltonian form: 
\begin{align}
\delta^2 S_E =&\int \dd{r} \bigg[
\Ppsi \dpsid + \PE \dEd + \Pf \Dot{f} + \Pdph \dphd \notag \\
&+ \frac{1}{4 \left(\triangle + 3 \kh\right) a^2}
\left( \kh \Ppsi^2
- \frac{3}{\triangle} \PE^2
- 2 \Ppsi \PE \right)
+ \frac{a^2}{2} e^{b \ph} \triangle \Pf^2
+ \frac{1}{2a^2}\Pdph^2
- \frac{1}{2} \phd \Ppsi \dph 
+ a^2 \left(\triangle + 3 \kh \right) \psi^2\notag \\
&+ \frac{e^{-b\ph}}{2a^2} \left(f + Q (3 \dpsi - \triangle \dE - b\dph) \right)^2 - \frac{e^{-b\ph}}{4a^2} Q^2 b^2 \dph^2 
+ \frac{1}{2a^2} \left( \frac{3}{2} (\phd)^2 - \triangle \right) \dph^2
- \dB \left( \PE + Q \triangle \Pf \right)\notag\\
&- \dA \left( \Pdph \phd - \Hh \Ppsi + \frac{Q \, e^{-b \ph}}{a^2} \left( Q( \triangle \dE - 3 \dpsi + \frac{1}{2} b \dph ) - f \right)
+ a^2 \left( 3 \Hh \phd \dph + 2 ( \triangle + 3 \kh ) \dpsi \right) \right) \bigg]
\end{align}
and gives rise to the two constraint equations:
\begin{align}
&\dA : \Pdph \phd - \Hh \Ppsi + \frac{Q \, e^{-b \ph}}{a^2} \left( Q( \triangle \dE - 3 \dpsi + \frac{1}{2} b \dph ) - f \right)
+ a^2 \left( 3 \Hh \phd \dph + 2 ( \triangle + 3 \kh ) \dpsi \right) = 0\\
&\dB : \PE + Q \triangle \Pf = 0.
\end{align}
In order to resolve gauge issues, we need to introduce gauge-invariant variables. In the three-form formalism of axions we have
\begin{align}
R &= f - Q \triangle E,& \Phi &= \dph + \frac{\psi}{\Hh} \phd
\end{align}
where $R$ is defined as in \cite{Loges:2022nuw} for the three-form fluctuations, while $\Phi$ is a gauge-invariant Mukhanov variable \cite{Garriga:1997wz,Gratton:2001gw}. The respective conjugate momenta are
\begin{align}\label{actionRphi}
\PR &= \Pf + \frac{Q e^{-b \ph}}{a^2 \Hh}\psi,&
\PPh &= \Pdph - \left(\frac{b e^{-b \ph}}{2a^2 \Hh} + 3 a^2 \phd  \right) \dpsi.
\end{align}
The quadratic action in terms of these gauge invariant variables
\begin{align}\label{gauge inv three-form hamiltonian}
\delta^2 S_E =&\int \dd{r} \Bigg[\PR \Dot{R} + \PPh \Dot{\Phi}
+ \PR \left(
- \frac{e^{-b \ph} Q^2 \triangle}{2 a^4 \Hh (\triangle + 3 \kh)} R
+ \frac{Q \triangle}{4(\triangle+3\kh)} \left(\frac{b e^{-b\ph}Q^2}{a^4 \Hh} + 6 \phd \right) \Phi
\right)\notag\\
&+ \PPh \left(
\frac{Q \triangle \phd}{2a^2 \Hh \left(\triangle + 3 \kh \right)} \PR
- \frac{e^{-b\ph} Q \kh \phd}{2 a^4 \Hh^2 (\triangle + 3 \kh)} R
+ \frac{\phd\left(b e^{-b \ph} Q^2 \kh- 2 a^4 \Hh \triangle  \phd \right)}{4 a^4 \Hh^2 (\triangle + 3 \kh)} \Phi
\right)\notag\\
&+ \frac{\triangle \left(-3Q^2 + 2 e^{b \ph} a^4 (\triangle + 3 \kh) \right)}{4 a^2 (\triangle + 3 \kh)} \PR^2
+ \frac{e^{-2 b \ph} \left(-Q^2 \triangle + e^{b \ph} a^4 (\triangle + 3 \kh) \left(6 \kh + (\phd)^2\right)\right)}{12 a^6 \Hh^2 (\triangle+3\kh)} R^2\notag\\
&+ \frac{e^{-2b\ph} \left( b Q^3 (2 \triangle +3 \kh) - 2 e^{b\ph} Q a^4 \left( - 3 \Hh \triangle \phd + b (\triangle + 3 \kh) (6 \kh + (\phd)^2)  \right) \right)}{12 a^6 \Hh^2 (\triangle + 3 \kh) } R \Phi \notag\\
&+\frac{e^{-2 b \ph}}{48 a^6 \Hh^2 (\triangle + 3 \kh)}\Big( - b^2 Q^4 (2\triangle + 3 \kh) - e^{2b\ph} \triangle a^8 (6 \kh + (\phd)^2) (2 (\triangle+3\kh) + 3 (\phd)^2)\notag\\
&+e^{b \ph} Q^2 a^4 (2(\triangle + 3 \kh) (\triangle + 3 b^2 \kh) - 6 b \triangle \Hh \phd + (3 \triangle + b^2 \triangle+ 3 b^2 \kh)(\phd)^2) \Big) \Phi^2\notag\\
&+\frac{e^{-b\ph} \left(Q^2 (\triangle + 3 \kh) - e^{b \ph} a^4 (6 \kh (\triangle + 3 \kh)+ \triangle (\phd)^2)\right)}{12 a^6 \Hh^2 (\triangle + 3 \kh)} \PPh^2
\Bigg].
\end{align}
This constitutes our sought-for quadratic action which depends only on two gauge-invariant variables and which has the constraints incorporated. 

\subsubsection{The scalar formulation}
Similarly, for the scalar description of the axion field, which is equivalent with the correct boundary conditions, when we combine the gravity sector with the field sector, we can simplify the resulting quadratic action by applying the equations of motion \eqref{eqn:equation-of-motion}. This yields, up to a total derivative in $r$ and a total derivative on the induced metric,
\begin{align}
\delta^2 S_E =\int \dd{r} \dd[3]{x} a^2 \sqrt{\gamma} \Bigg[& e^{b \ph} \Big(
- \frac{1}{2} \left( \dchd^2 - \dch \triangle \dch \right) 
+ \chid \dchd \left( \dA - b \dph \right)
- \chid \dch \left( 3 \dpsid +\triangle ( \dB - \dEd \right)
+ \frac{1}{4} b \chid^2 \left( 2 \dA - b \dph \right) 
\Big) \notag\\
& +\frac{1}{2} \left( (\dphd)^2 - \dph \triangle \dph \right)
+ \phd \dph \left(3 \dpsid + \triangle \left( \dB - \dEd \right) \right) - \dA \phd \dphd \notag\\
&+ \dpsi \triangle \left(\dpsi - 2 \dA \right)
- 3 (\dpsid)^2 - 6 \Hh \dA \dpsid - 2 \left( \Hh \dA + \dpsid \right) \triangle \left( \dB - \dEd\right) \notag\\
&+ \kh \left( 3\dpsi^2 - 6 \dA \dpsi - 3 \dA^2 + \left(\dB - \dEd \right)\triangle \left(\dB - \dEd \right) \right)
\bigg]
\end{align}
The conjugate momenta of the dynamical variables $\psi, \dE, \chi \text{ and } \ph$ are given by
\begin{align}
\Pdch &= e^{b \ph} a^2 \left( A \chid - b \dph \chid - \dchd \right) ,&
\Ppsi &= a^2 \left( 3 \phd \dphd - 3 e^{b \ph} \chid \dch - 6 \dA \Hh - 6 \dpsid + 2 \triangle\left( \dEd - \dB \right)  \right), \notag\\
\Pdph &= a^2 \left( \dphd - \phd \dA \right),&
\PE &= \triangle a^2 \left( - \phd \dphd - e^{b \ph} \chid \dchd + 2 \dA \Hh + 2 \dpsid + 2 \kh \left( \dEd - \dB \right) \right).
\end{align}
When substituted into the action, this yields the action in Hamiltonian form 
\begin{align}\label{hamiltonian scalar field}
\delta^2 S_E =&\int \dd{r} \bigg[\Ppsi \dpsid + \PE \dEd + \Pdch \dchd + \Pdph \dphd \notag\\
&+ \frac{1}{4 \left(\triangle + 3 \kh\right) a^2}
\left( \kh \Ppsi^2
- \frac{3}{\triangle} \PE^2
- 2 \Ppsi \PE \right)
+ \frac{1}{2 a^2} e^{- b \ph} \Pdch^2
+ \frac{1}{2 a^2}\Pdph^2
+ \Pdch b \dph \chid 
- \frac{1}{2} \Ppsi \left( \phd \dph - e^{b \ph} \chid \dch \right)\notag \\
&+ a^2 \left(\triangle + 3 \kh \right) \psi^2
+ \frac{1}{2} a^2 \left( \left( \triangle + \frac{3}{2} e^{b \ph} \chid^2 \right) \dch^2
+ \left(  \triangle - \frac{3}{2} \phd^2 - b^2 e^{b \ph} \chid^2 \right) \dph^2
- 3 e^{b \ph} \phd \dph \chid \dch \right)\notag\\
&- \dB \PE - \dA \left( \Pdph \phd + \Pdch \chid - \Hh \Ppsi +
+ a^2 \left( 3 \Hh \phd \dph - 3 \Hh e^{b \ph} \chid \dchd - \frac{1}{2} b e^{b \ph} \chid^2 + 2 ( \triangle + 3 \kh ) \dpsi \right) \right) \bigg]
\end{align}
and two constraints:
\begin{align}
&\dA :  \Pdph \phd + \Pdch \chid - \Hh \Ppsi +
+ a^2 \left( 3 \Hh \phd \dph - 3 \Hh e^{b \ph} \chid \dchd - \frac{1}{2} b e^{b \ph} \chid^2 + 2 ( \triangle + 3 \kh ) \dpsi \right) = 0\\
&\dB : \PE = 0.
\end{align}


We now introduce the following gauge invariant variables
\begin{align}
\Chi &= \dch + \frac{\psi}{\Hh} \chid, & \Phi &= \dph + \frac{\psi}{\Hh} \phd.
\intertext{The respective conjugate momenta are}
\PCh &= \Pdch + 3 e^{b \ph} a^2 \chid \dpsi,&
\PPh &= \Pdph - \left(\frac{b e^{-b \ph}}{2a^2 \Hh} + 3 a^2 \phd  \right) \dpsi.
\end{align}
In terms of these gauge invariant variables, the quadratic action reads:
\begin{align}\label{scalar hamiltonian}
\delta^2 S_E =&\int \dd{r} \Bigg[\PCh \Dot{\Chi} + \PPh \Dot{\Phi}
+ \Chi \left(
  \frac{e^{b \ph} \chid^2 \triangle}{2 \Hh (\triangle + 3 \kh)} \PCh
+ \frac{e^{b \ph} \chid \triangle a^2}{4(\triangle+3\kh)} \left(\frac{b e^{b\ph} \chid^2}{\Hh} + 6 \phd \right) \Phi
\right)\notag\\
&+ \PPh \left(
\frac{e^{b \ph} \triangle \chid \phd}{2 \Hh \left(\triangle + 3 \kh \right)} \Chi
+ \frac{\kh \chid \phd}{2 a^2 \Hh^2 (\triangle + 3 \kh)} \PCh
+ \frac{\phd \left(b e^{b \ph} \chid^2 \kh - 2 \Hh \triangle  \phd \right)}{4 \Hh^2 (\triangle + 3 \kh)} \Phi
\right)\notag\\
&+ \frac{ e^{b \ph} a^2 \triangle \left( 2 (\triangle + 3 \kh) - 3 e^{b \ph} \chid^2 \right)}{4 (\triangle + 3 \kh)} \Chi^2
+ \frac{e^{- b \ph} \left( (\triangle + 3 \kh) \left(6 \kh + \phd^2 \right)-e^{b \ph} \triangle \chid^2 \right)}{12 a^2 \Hh^2 (\triangle+3\kh)} \PCh^2\notag\\
&-\frac{ \left( b e^{b\ph} \chid^2 (2 \triangle +3 \kh)  - 2 \chid \left( - 3 \Hh \triangle \phd + b (\triangle + 3 \kh) (6 \kh + (\phd)^2)  \right) \right)}{12 \Hh^2 (\triangle + 3 \kh) } \PCh \Phi \notag\\
&+\frac{a^2}{48 \Hh^2 (\triangle + 3 \kh)}\big( - b^2 e^{2 b \ph} \chid^4 (2\triangle + 3 \kh) - \triangle (6 \kh + (\phd)^2) (2 (\triangle+3\kh) + 3 (\phd)^2)\notag\\
&+ 2 e^{b\ph} \chid^2 (2(\triangle + 3 \kh) (\triangle + 3 b^2 \kh) - 6 b \triangle \Hh \phd + \phd^2 (3 \triangle + b^2 \triangle + 3 b^2 \kh)) \big) \Phi^2\notag\\
&-\frac{ \left( (\triangle + 3 \kh) (6 \kh -e^{b\ph} \chid^2) + \triangle (\phd)^2)\right)}{12 a^2 \Hh^2 (\triangle + 3 \kh)} \PPh^2
\Bigg].
\end{align}
Applying the substitution of $\chid$ from \eqref{transformations axion} and a symplectic transformation (including the $\PCh \Chi$ boundary term)
\begin{align}
\Chi &\to \PR,& \PCh &\to - R,
\end{align}
we recover exactly the same quadratic action as in \eqref{gauge inv three-form hamiltonian}, as expected.

We can confirm the conclusions from Section \ref{stabilitysec} related to the boundary conditions on $\Chi$. Rewriting the charge fluctuations using \eqref{transformations axion} we find
\begin{align}\label{charge fluctuations in terms of momenta}
\delta Q_\text{axion} = \int_{S^3} \dd[3]{x} \sqrt{\gamma} \left[ a^2 e^{b\ph} \dchd - Q\left( 3 \dpsi + \dA - \triangle \dE-b\dph \right) \right] = - \int_{S^3} \dd[3]{x} \sqrt{\gamma} \, \PCh,
\end{align}
where the total derivative on the three-sphere vanishes upon integration. Therefore, Dirichlet boundary conditions of axion-charge fluctuations thus translate to sets a Neumann condition on $\Chi$ or equivalently a Dirichlet boundary condition on its conjugate momentum $\PCh$, as discussed before.

